s-process Enriched Post-AGB Star J003643.94-723722.1 in the SMC with an Extreme C/O Ratio and the First Precise Detection of Lead

Post-asymptotic giant branch (post-AGB) stars are exquisite tracers of s-process nucleosynthesis via their surface abundances. We present a comprehensive analysis of J003643.94$-$723722.1 (J003643), a single SMC post-AGB star, using high-resolution UVES/VLT spectra analysed with E-iSpec. We find C/O = 16.21 and $[\mathrm{s}/\mathrm{Fe}]=2.09\pm0.20 \mathrm{dex}$. We also report the first direct Pb detection in a post-AGB star from the Pb II 5608.853 A line, with $[\mathrm{Pb}/\mathrm{Fe}]=3.18\,\mathrm{dex}$. Comparison with post-AGB samples in the Galaxy and Magellanic Clouds reveals that J003643 has an unusually high C/O ratio. J003643's $[\mathrm{C}/\mathrm{Fe}]=1.33\pm0.14 \mathrm{dex}$ and $[\mathrm{s}/\mathrm{Fe}]=2.09\pm0.20\,\mathrm{dex}$ are consistent with third dredge-up enrichment, but its $[\mathrm{O}/\mathrm{Fe}]=-0.08\pm0.20\,\mathrm{dex}$ is low relative to objects of similar $[\mathrm{C}/\mathrm{Fe}]$ and $[\mathrm{Fe}/\mathrm{H}]$. Together with $[\alpha/\mathrm{Fe}]\approx0\,\mathrm{dex}$ at $[\mathrm{Fe}/\mathrm{H}]\approx-1\,\mathrm{dex}$, consistent with SMC chemical evolution, this indicates the high C/O chiefly reflects oxygen deficiency rather than exceptional carbon enrichment. Additionally, we compare the full abundance pattern with yields from ATON, MONASH and FRUITY (the latter two with post-processing nucleosynthesis). Most elements are reproduced, but Pb is strongly underpredicted, highlighting a persistent gap in models of heavy-element production in AGB stars. The photospheric chemistry of J003643 adds to the growing diversity among post-AGB stars and underscores the complexity of AGB nucleosynthesis.

==> Null.tex <==
%Table 2

\begin{landscape}
    \begin{table}
        \caption{Photometric data of the targets. See text for full details.}
        \begin{center}
            \resizebox{\linewidth}{!}{%
            \begin{tabular}{ c c c c c c c c c c c c c c c c c c c c c }
            \hline
            Object Name & RA ($\degree$) & Dec ($\degree$) & U & B & SDSS.RP & V & R & I & J & H & K & W1 & W2 & AKARI.S9W & IRAS.F12 & W3 & W4 & IRAS.F25 & IRAS.F60 & IRAS.F100\\
            \hline
            J005107  & 12.780083 & -73.692598 & 16.65 & 16.657 & 99.99 & 15.84 & 15.45 & 14.85 & 14.33 & 13.65 & 12.93 & 11.39 & 10.44 & 99.99 & 99.99 & 8.365 & 6.926 & 99.99 & 99.99 & 99.99 \\
            MACHO 47.2496.8  & 73.930267 & -67.852718 & 17.31 & 16.23 & 99.99 & 15.08 & 14.28 & 14.00 & 13.19 & 12.67 & 12.57 & 12.09 & 11.79 & 99.99 & 99.99 & 10.26 & 9.248 & 99.99 & 99.99 & 99.99 \\
            HD 158616 & 262.695520 & -11.368968 & 11.92 & 10.09 & 9.368 & 9.642 & 99.99 & 99.99 & 7.845 & 7.299 & 6.525 & 5.178 & 4.029 & 3.301 & 3.520 & 2.600 & 1.234 & 2.900 & 1.600 & 1.980 \\
            V453 Oph  & 261.704705 & -2.393453 & 12.29 & 11.90 & 10.30 & 10.85 & 10.50 & 9.791 & 8.806 & 8.442 & 8.283 & 7.993 & 7.890 & 99.99 & 99.99 & 7.743 & 7.549 & 99.99 & 99.99 & 99.99 \\
            \hline
            \end{tabular}
            }
        \end{center}
        \begin{tablenotes}
        
        \small
    \item \textbf{Notes:} The RA and DEC coordinates are given for the J2000 epoch. Null magnitudes are listed as 99.999.
        \end{tablenotes}
       
        \label{tab:photometry}
    \end{table}    ,
\end{landscape}




%Table 1

\begin{landscape}
    \begin{table}
        \caption{This table lists the object name and alternative widely used name for each object in the sample along with two sets of stellar parameters. The final column lists the references to the literature analysis.}
        \begin{center}
            \begin{tabular}{ c l l c c c c c c c c c c  }
                \hline
            \#ID & Object Name & Other Name & \begin{tabular}[c]{@{}l@{}}\Teff\\ {(}K{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\logg \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\feh \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\mv \\ {(}dex{)}\end{tabular} & & \begin{tabular}[c]{@{}l@{}}\Teff \\ {(}K{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\logg \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\feh \\ {(}dex{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\mv \\ {(}dex{)}\end{tabular} & Ref. \\
                \hline
        		\multicolumn{3}{ c }{} & \multicolumn{4}{c }{This Study} & \multicolumn{5}{c }{Literature} \\
                \hline
                1 & J005107.19-734133.3 &	OGLE SMC-T2CEP-18	& 5768 $\pm$ 100	&	0.21 $\pm$ 0.10	&	-1.57 $\pm$ 0.10   &	4.08 $\pm$ 0.50	& & 5267 $\pm$ 250	&	0.72 $\pm$ 0.50	&	-1.56 $\pm$ 0.50  & ... & 1	\\
                2 & MACHO 47.2496.8 &	OGLE LMC-T2CEP-15	&
                4898 $\pm$ 100	&	0.00 $\pm$ 0.50	&	-1.42 $\pm$ 0.16   &	4.00 $\pm$ 1.00	& & 4900 $\pm$ 250	&	0.00 $\pm$ 0.50	&	-1.50 $\pm$ 0.50   &	3.50 $\pm$ 1.00  &	2\\
                3 & HD 158616 &	IRAS 17279-1119	& 7379 $\pm$ 110	&	1.47 $\pm$ 0.25	&	-0.50 $\pm$ 0.20   &	2.97 $\pm$ 0.25 &  & 7250 $\pm$ 125	&	1.25 $\pm$ 0.25	&	-0.64 $\pm$ 0.12 &	3.00 $\pm$ 0.50 &	3\\
                4 & V453 Oph &	BD-02 4345	& 	6158 $\pm$ 100	&	1.19 $\pm$ 0.25	&	-2.27 $\pm$ 0.10   &	2.50 $\pm$ 0.50 &  & 6250 $\pm$ 250	&	1.50 $\pm$ 0.50	&	-2.23 $\pm$ 0.12   &	3.00 $\pm$ 0.50 & 4\\
                \hline
            \end{tabular}
        \end{center}
        \begin{tablenotes}
        
        \small
    \item \textbf{Notes:} The stellar parameters under "This study" represent the spectroscopically determined atmospheric parameters obtained using the $Python$ wrapper of i-Spec whereas the stellar parameters under the title "Literature" represent the spectroscopically determined atmospheric parameters from the Literature analysis. Note that the low-resolution spectral analysis of J005107.19-734133.3 did not provide an estimated \mv value. Detailed information on the tabulated information can be found in the individual studies identified in column 'Ref'. The column 'Ref.' indicates the individual study: 1 - \cite{Kamath2014}, 2 - \cite{Reyniers2007}, 3 - \cite{desmedt2016}, 4 - \cite{Deero2005}\\
        \end{tablenotes}
       
        \label{tab:sample}
    \end{table}    ,
\end{landscape}


==> Supplementary_Material.tex <==
\begin{table}
    \centering
    \caption{Linelist of J003643}
        \label{tab:linelistFull_J003643}
        \begin{tabular}{ c c c c c c c c }
            \hline
            \addlinespace
            Ion & wavelength (\AA) & log gf & EP(eV) & EW (m\AA) \\
            \addlinespace
            \hline
            \addlinespace
            C 1 & 4812.917 & -3.377 & 7.48 & 15.50 \\
            C 1 & 4932.049 & -1.658 & 7.685 & 144.80 \\
            C 1 & 5017.086 & -2.457 & 7.946 & 43.90 \\
            C 1 & 5024.919 & -2.728 & 7.946 & 22.40 \\
            C 1 & 5039.057 & -1.79 & 7.946 & 100.40 \\
            C 1 & 5057.681 & -2.223 & 8.647 & 22.80 \\
            C 1 & 5153.569 & -2.187 & 8.647 & 31.00 \\
            C 1 & 5380.325 & -1.616 & 7.685 & 143.40 \\
            C 1 & 5547.265 & -2.253 & 8.64 & 20.80 \\
            C 1 & 6002.98 & -2.169 & 8.647 & 17.00 \\
            C 1 & 6007.173 & -2.062 & 8.64 & 20.40 \\
            C 1 & 6010.672 & -1.938 & 8.64 & 25.70 \\
            C 1 & 6013.167 & -1.314 & 8.647 & 77.80 \\
            C 1 & 6014.833 & -1.584 & 8.643 & 48.50 \\
            O 1 & 6155.971 & -0.67 & 10.74 & 9.50 \\
            O 1 & 6156.755 & -0.452 & 10.741 & 13.60 \\
            O 1 & 6158.187 & -0.296 & 10.741 & 19.10 \\
            Mg 1 & 5172.684 & -0.45 & 2.712 & 200.10 \\
            Mg 1 & 5528.405 & -0.498 & 4.346 & 56.00 \\
            Ca 1 & 5857.451 & 0.24 & 2.933 & 22.40 \\
            Ca 1 & 6122.217 & -0.316 & 1.886 & 34.90 \\
            Ca 1 & 6162.173 & -0.09 & 1.899 & 45.50 \\
            Ca 1 & 6439.075 & 0.39 & 2.526 & 33.30 \\
            Ca 2 & 5001.479 & -0.507 & 7.505 & 15.00 \\
            Ca 2 & 5019.971 & -0.247 & 7.515 & 24.30 \\
            Sc 2 & 5031.021 & -0.4 & 1.357 & 63.00 \\
            Sc 2 & 5526.79 & 0.024 & 1.768 & 83.10 \\
            Ti 2 & 4805.085 & -0.96 & 2.061 & 97.50 \\
            Ti 2 & 4911.194 & -0.64 & 3.124 & 50.90 \\
            Ti 2 & 5013.686 & -2.14 & 1.582 & 27.10 \\
            Ti 2 & 5072.286 & -1.02 & 3.124 & 20.10 \\
            Ti 2 & 5129.156 & -1.34 & 1.892 & 63.70 \\
            Ti 2 & 5154.068 & -1.75 & 1.566 & 62.00 \\
            Ti 2 & 5185.902 & -1.41 & 1.893 & 62.70 \\
            Ti 2 & 5188.687 & -1.05 & 1.582 & 139.30 \\
            Ti 2 & 5211.53 & -1.41 & 2.59 & 20.70 \\
            Ti 2 & 5262.141 & -2.25 & 1.582 & 34.00 \\
            Ti 2 & 5268.608 & -1.61 & 2.598 & 23.20 \\
            Ti 2 & 5336.786 & -1.6 & 1.582 & 61.80 \\
            Ti 2 & 5381.022 & -1.97 & 1.566 & 53.80 \\
            Ti 2 & 5418.768 & -2.13 & 1.582 & 25.70 \\
            Cr 1 & 5204.498 & -0.19 & 0.941 & 29.90 \\
            Cr 1 & 5208.409 & 0.17 & 0.941 & 85.70 \\
            Cr 2 & 5232.496 & -2.36 & 4.071 & 13.80 \\
            Cr 2 & 5237.328 & -1.35 & 4.073 & 63.30 \\
            Cr 2 & 5274.964 & -1.559 & 4.071 & 46.00 \\
            Cr 2 & 5305.853 & -2.16 & 3.827 & 24.60 \\
            Cr 2 & 5313.563 & -1.779 & 4.074 & 47.90 \\
            Cr 2 & 5334.869 & -1.826 & 4.072 & 26.10 \\
            Cr 2 & 5407.604 & -2.151 & 3.827 & 18.90 \\
            Cr 2 & 5420.922 & -2.458 & 3.758 & 10.90 \\
            Cr 2 & 5478.365 & -1.968 & 4.178 & 18.00 \\
            Fe 1 & 4938.814 & -1.077 & 2.876 & 15.10 \\
            Fe 1 & 4957.596 & 0.233 & 2.808 & 112.90 \\
            Fe 1 & 4982.499 & 0.156 & 4.103 & 20.20 \\
            Fe 1 & 4983.853 & -0.006 & 4.103 & 14.40 \\
            Fe 1 & 5001.863 & 0.01 & 3.882 & 28.30 \\
            Fe 1 & 5005.712 & 0.029 & 3.884 & 24.70 \\
            Fe 1 & 5006.119 & -0.638 & 2.833 & 36.20 \\
            Fe 1 & 5049.82 & -1.355 & 2.279 & 20.90 \\
            Fe 1 & 5065.018 & 0.005 & 4.256 & 15.40 \\
            Fe 1 & 5068.766 & -1.042 & 2.94 & 14.70 \\
            Fe 1 & 5125.117 & -0.14 & 4.22 & 11.30 \\
            Fe 1 & 5139.251 & -0.741 & 2.998 & 26.40 \\
            Fe 1 & 5139.462 & -0.509 & 2.94 & 47.20 \\
            Fe 1 & 5162.273 & 0.02 & 4.178 & 22.40 \\
            Fe 1 & 5171.596 & -1.793 & 1.485 & 39.10 \\
            Fe 1 & 5194.941 & -2.09 & 1.557 & 19.00 \\
            Fe 1 & 5232.94 & -0.058 & 2.94 & 68.00 \\
            Fe 1 & 5266.555 & -0.386 & 2.998 & 36.10 \\
            Fe 1 & 5269.537 & -1.321 & 0.859 & 120.60 \\
            Fe 1 & 5270.356 & -1.339 & 1.608 & 76.90 \\
            Fe 1 & 5281.79 & -0.834 & 3.039 & 16.10 \\
            Fe 1 & 5283.621 & -0.432 & 3.241 & 32.80 \\
            Fe 1 & 5328.039 & -1.466 & 0.915 & 92.80 \\
            Fe 1 & 5328.531 & -1.85 & 1.557 & 25.10 \\
            Fe 1 & 5341.024 & -1.953 & 1.608 & 23.30 \\
            Fe 1 & 5364.871 & 0.228 & 4.446 & 24.40 \\
            Fe 1 & 5367.466 & 0.443 & 4.415 & 28.20 \\
            Fe 1 & 5369.961 & 0.536 & 4.371 & 35.10 \\
            Fe 1 & 5371.489 & -1.645 & 0.958 & 65.50 \\
            Fe 1 & 5383.368 & 0.645 & 4.313 & 38.60 \\
            Fe 1 & 5397.128 & -1.993 & 0.915 & 48.00 \\
            Fe 1 & 5404.151 & 0.523 & 4.435 & 41.50 \\
            Fe 1 & 5405.775 & -1.844 & 0.99 & 45.20 \\
            Fe 1 & 5410.91 & 0.398 & 4.473 & 23.40 \\
            Fe 1 & 5415.199 & 0.642 & 4.387 & 34.40 \\
            Fe 1 & 5424.068 & 0.52 & 4.32 & 41.30 \\
            Fe 1 & 5434.524 & -2.122 & 1.011 & 33.70 \\
            Fe 1 & 5463.275 & 0.11 & 4.435 & 16.80 \\
            Fe 1 & 5569.618 & -0.486 & 3.417 & 13.00 \\
            Fe 1 & 5572.842 & -0.275 & 3.397 & 22.20 \\
            Fe 1 & 5586.756 & -0.12 & 3.368 & 34.00 \\
            Fe 1 & 5615.644 & 0.05 & 3.332 & 50.40 \\
            Fe 1 & 6136.615 & -1.4 & 2.453 & 10.40 \\
            Fe 1 & 6137.691 & -1.403 & 2.588 & 7.40 \\
            Fe 1 & 6191.557 & -1.417 & 2.433 & 11.10 \\
            Fe 1 & 6393.6 & -1.432 & 2.433 & 7.80 \\
            Fe 2 & 5136.795 & -4.29 & 2.844 & 18.10 \\
            Fe 2 & 5234.623 & -2.23 & 3.221 & 151.70 \\
            Fe 2 & 5256.932 & -4.182 & 2.891 & 18.40 \\
            Fe 2 & 5275.997 & -1.94 & 3.199 & 186.30 \\
            Fe 2 & 5337.722 & -3.788 & 3.23 & 31.20 \\
            Ni 1 & 5080.533 & 0.32 & 3.655 & 10.20 \\
            Y 2 & 4982.13 & -1.29 & 1.033 & 62.00 \\
            Y 2 & 5119.112 & -1.36 & 0.992 & 62.40 \\
            Y 2 & 5196.422 & -1.27 & 1.748 & 39.50 \\
            Y 2 & 5200.41 & -0.57 & 0.992 & 151.60 \\
            Y 2 & 5402.774 & -0.63 & 1.839 & 111.20 \\
            Y 2 & 5473.385 & -1.02 & 1.738 & 70.80 \\
            Y 2 & 5480.73 & -0.99 & 1.721 & 64.70 \\
            Y 2 & 5497.406 & -0.58 & 1.748 & 135.30 \\
            Y 2 & 5521.562 & -0.933 & 1.738 & 53.80 \\
            Y 2 & 5544.611 & -1.09 & 1.738 & 70.40 \\
            Y 2 & 5546.009 & -1.1 & 1.748 & 84.10 \\
            Y 2 & 5728.886 & -1.12 & 1.839 & 48.80 \\
            Y 2 & 6613.732 & -1.11 & 1.748 & 65.30 \\
            Y 2 & 6795.416 & -1.03 & 1.738 & 59.60 \\
            Zr 2 & 5112.27 & -0.85 & 1.665 & 83.60 \\
            Zr 2 & 5350.089 & -1.24 & 1.827 & 66.30 \\
            Zr 2 & 5350.35 & -1.16 & 1.773 & 68.20 \\
            La 2 & 4809 & -1.4 & 0.235 & 59.70 \\
            La 2 & 4970.39 & -1.16 & 0.321 & 70.00 \\
            La 2 & 4986.82 & -1.3 & 0.173 & 77.40 \\
            La 2 & 4999.46 & -0.77 & 0.403 & 146.70 \\
            La 2 & 5114.56 & -1.03 & 0.235 & 109.40 \\
            La 2 & 5156.73 & -1.85 & 0.126 & 30.10 \\
            La 2 & 5157.433 & -0.33 & 2.21 & 26.40 \\
            La 2 & 5163.61 & -1.81 & 0.244 & 26.60 \\
            La 2 & 5259.38 & -1.95 & 0.173 & 26.10 \\
            La 2 & 5290.82 & -1.65 & 0 & 36.30 \\
            La 2 & 5302.582 & -0.52 & 2.058 & 31.20 \\
            La 2 & 5303.53 & -1.35 & 0.321 & 55.60 \\
            La 2 & 5377.052 & -0.43 & 2.304 & 25.10 \\
            La 2 & 5535.656 & -1.25 & 1.252 & 19.40 \\
            La 2 & 5863.69 & -1.37 & 0.927 & 11.00 \\
            La 2 & 6129.556 & -1.5 & 0.772 & 17.30 \\
            La 2 & 6320.376 & -1.61 & 0.173 & 55.70 \\
            La 2 & 6390.48 & -1.41 & 0.321 & 62.20 \\
            Ce 2 & 4914.924 & -0.81 & 0.879 & 29.80 \\
            Ce 2 & 4971.494 & 0.34 & 1.786 & 51.80 \\
            Ce 2 & 4984.433 & -1.02 & 1.027 & 10.60 \\
            Ce 2 & 4986.385 & -1.05 & 1.026 & 20.10 \\
            Ce 2 & 5011.759 & -0.49 & 1.048 & 52.90 \\
            Ce 2 & 5022.867 & -0.38 & 1.044 & 43.30 \\
            Ce 2 & 5039.801 & -0.41 & 1.615 & 18.90 \\
            Ce 2 & 5044.023 & -0.14 & 1.212 & 53.30 \\
            Ce 2 & 5075.355 & -0.35 & 1.026 & 61.30 \\
            Ce 2 & 5077.854 & -0.48 & 1.412 & 17.50 \\
            Ce 2 & 5079.682 & 0.42 & 1.384 & 93.40 \\
            Ce 2 & 5117.169 & -0.05 & 1.402 & 46.60 \\
            Ce 2 & 5147.565 & -0.3 & 1.279 & 27.90 \\
            Ce 2 & 5187.458 & 0.17 & 1.212 & 87.80 \\
            Ce 2 & 5252.662 & -0.64 & 1.155 & 29.20 \\
            Ce 2 & 5265.676 & -0.23 & 1.247 & 57.70 \\
            Ce 2 & 5274.229 & 0.13 & 1.044 & 97.50 \\
            Ce 2 & 5330.556 & -0.4 & 0.869 & 61.20 \\
            Ce 2 & 5353.524 & 0.09 & 0.879 & 108.50 \\
            Ce 2 & 5409.229 & -0.29 & 1.103 & 52.00 \\
            Ce 2 & 5459.193 & -0.33 & 1.615 & 23.30 \\
            Ce 2 & 5468.371 & -0.07 & 1.402 & 37.00 \\
            Ce 2 & 5472.279 & -0.1 & 1.247 & 42.80 \\
            Ce 2 & 5518.489 & -0.65 & 1.155 & 20.50 \\
            Ce 2 & 5623.001 & -1.15 & 0.956 & 13.60 \\
            Ce 2 & 5975.818 & -0.45 & 1.327 & 29.60 \\
            Ce 2 & 6043.373 & -0.48 & 1.206 & 34.00 \\
            Pr 2 & 5034.406 & -0.09 & 1.111 & 15.70 \\
            Pr 2 & 5110.763 & 0.32 & 1.148 & 32.50 \\
            Pr 2 & 5129.536 & -0.134 & 0.648 & 28.10 \\
            Pr 2 & 5173.902 & 0.384 & 0.968 & 37.80 \\
            Pr 2 & 5206.555 & -0.06 & 0.95 & 10.70 \\
            Pr 2 & 5292.619 & -0.257 & 0.648 & 15.60 \\
            Nd 2 & 4811.342 & -1.14 & 0.064 & 58.30 \\
            Nd 2 & 4902.037 & -1.34 & 0.064 & 19.30 \\
            Nd 2 & 4930.725 & -1.16 & 0.823 & 20.70 \\
            Nd 2 & 4959.119 & -0.8 & 0.064 & 50.50 \\
            Nd 2 & 4961.387 & -0.71 & 0.631 & 43.60 \\
            Nd 2 & 4987.16 & -0.79 & 0.742 & 29.00 \\
            Nd 2 & 4989.95 & -0.5 & 0.631 & 56.20 \\
            Nd 2 & 4998.541 & -1.1 & 0.471 & 38.10 \\
            Nd 2 & 5000.43 & -1.31 & 0.321 & 26.60 \\
            Nd 2 & 5033.51 & -0.47 & 1.136 & 28.00 \\
            Nd 2 & 5063.72 & -0.62 & 0.976 & 24.50 \\
            Nd 2 & 5076.58 & -0.25 & 0.742 & 92.40 \\
            Nd 2 & 5089.832 & -1.16 & 0.205 & 26.60 \\
            Nd 2 & 5092.79 & -0.61 & 0.38 & 53.60 \\
            Nd 2 & 5105.23 & -0.61 & 1.136 & 24.90 \\
            Nd 2 & 5123.78 & -0.61 & 0.38 & 55.80 \\
            Nd 2 & 5130.59 & 0.45 & 1.304 & 87.20 \\
            Nd 2 & 5132.33 & -0.71 & 0.559 & 37.60 \\
            Nd 2 & 5165.13 & -0.74 & 0.68 & 29.70 \\
            Nd 2 & 5176.78 & -0.84 & 1.121 & 22.60 \\
            Nd 2 & 5181.169 & -0.6 & 0.859 & 28.00 \\
            Nd 2 & 5182.59 & -0.91 & 0.745 & 30.50 \\
            Nd 2 & 5212.36 & -0.96 & 0.205 & 35.30 \\
            Nd 2 & 5228.42 & -1.28 & 0.38 & 23.00 \\
            Nd 2 & 5249.58 & 0.2 & 0.976 & 102.50 \\
            Nd 2 & 5255.506 & -0.67 & 0.205 & 59.90 \\
            Nd 2 & 5273.43 & -0.18 & 0.68 & 82.40 \\
            Nd 2 & 5293.16 & 0.1 & 0.823 & 103.00 \\
            Nd 2 & 5306.46 & -0.97 & 0.859 & 18.80 \\
            Nd 2 & 5319.81 & -0.14 & 0.55 & 92.10 \\
            Nd 2 & 5356.97 & -0.28 & 1.264 & 38.10 \\
            Nd 2 & 5361.467 & -0.37 & 0.68 & 63.60 \\
            Nd 2 & 5371.93 & 0 & 1.412 & 43.90 \\
            Nd 2 & 5385.888 & -0.82 & 0.742 & 21.80 \\
            Nd 2 & 5416.374 & -0.93 & 0.859 & 12.10 \\
            Nd 2 & 5431.52 & -0.47 & 1.121 & 28.60 \\
            Nd 2 & 5485.7 & -0.12 & 1.264 & 39.60 \\
            Nd 2 & 5533.82 & -1.23 & 0.559 & 13.60 \\
            Nd 2 & 5708.271 & -0.58 & 0.859 & 41.00 \\
            Nd 2 & 5718.12 & -0.4 & 1.41 & 23.70 \\
            Sm 2 & 4913.26 & -0.93 & 0.659 & 13.10 \\
            Sm 2 & 4961.94 & -1.09 & 0.434 & 14.60 \\
            Sm 2 & 5052.75 & -0.16 & 1.376 & 26.00 \\
            Sm 2 & 5103.09 & -0.35 & 1.166 & 21.60 \\
            Sm 2 & 5116.69 & -0.72 & 0.933 & 13.80 \\
            Eu 2 & 6437.631 & -0.602 & 1.32 & 7.00 \\
            Eu 2 & 6645.094 & -0.162 & 1.38 & 23.70 \\
            Gd 2 & 5092.249 & -0.23 & 1.727 & 11.00 \\
            Gd 2 & 5108.903 & -0.36 & 1.659 & 12.90 \\
            Dy 2 & 4957.35 & -1.09 & 0 & 98.40 \\
            Er 2 & 5179.491 & 0.483 & 3.323 & 10.10 \\
            Yb 2 & 5335.159 & -0.26 & 3.789 & 15.90 \\
            Lu 2 & 4994.126 & -1.14 & 1.542 & 22.50 \\
            Hf 2 & 5040.812 & -1.42 & 1.482 & 39.30 \\
            Hf 2 & 5298.04 & -1.26 & 1.891 & 24.00 \\
            Pb 2 & 5608.853 & 0.2 & 7.371 & 12.10 \\
            \addlinespace
            \hline
        \end{tabular}
    \begin{center}
    \begin{tablenotes}
     \small
    \item \textbf{Notes:} Linelist used for the abundance determination of J003643. The last column shows the calculated equivalent width (EW). 
    \end{tablenotes}
    \end{center}  
\end{table}



==> Table5.tex <==
\begin{table*}
    \centering
    \caption{Luminosity of J003643 derived using the SED fitting method.}
        \label{tab:lum}
        \begin{tabular}{ c c c c c c}
            \hline
            \addlinespace
            \begin{tabular}[c]{@{}l@{}}\Lsed\\ {(}\Lsun{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\Delta$\Lsed\\ {(}\Lsun{)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}$E(B-V)$\\ {(}mag{)}\end{tabular} & SED type & Initial Mass \\
            \addlinespace
            \hline
            \addlinespace
            7623 & $^{+8606}_{-5761}$ & $0.46^{+0.50}_{-0.36}$ & Shell & 2$M_\odot$\\ 
            \addlinespace
            \hline
        \end{tabular}
    \begin{center}
    \begin{tablenotes}
     \small
    \item \textbf{Notes:} The luminosities derived from SED along with their corresponding upper and lower limits are displayed in Col. 1 and 2 respectively. The reddening derived from the SED model along with their corresponding upper and lower limits are shown in Col. 3 (see text for details). The initial mass estimate in Col. 5 is discussed in Section~\ref{sec:aton}. 
    \end{tablenotes}
    \end{center}  
\end{table*}

==> Table7_old.tex <==
\begin{sidewaystable}
    %\vspace*{0.35\textwidth}
    \captionsetup{justification=raggedright,singlelinecheck=false}
    \caption{LTE and NLTE abundance ratios of lead (\pbls\ and \pbhs) for \sprocess-rich single and binary post-AGB stars in the Galaxy and Magellanic Clouds, where lead abundance measurements are available. The table also includes their effective temperature and metallicity. See text for details.}
    \resizebox{\linewidth}{!}{%
    \centering
        \begin{tabular}{ c c c c c c c c c c c c c c c}
            \hline
            \addlinespace
             Index & Object name & LMC/SMC/Galaxy & 
             \Teff & \feh & <\logepsilon Pb I & \pbIfe & \logepsilon Pb II & \pbIIfe & \pbhs & \pbls & NLTE Std \pbhs & NLTE Std \pbls  & NLTE no H \pbhs & NLTE no H \pbls \\
             \hline
            \addlinespace
            1 &  J003643  &  SMC  &  7552 $\pm$ 91  &  -0.92 $\pm$ 0.11  &  ...  &  ...  & 4.29 & 3.58 & 1.39 & 1.865 &  ...  &  ...  &  ...  &  ... \\
            2 &  J004441.04-732136.4  &  SMC  &  6250 $\pm$ 125  &  -1.34 $\pm$ 0.32  &  <3  &  <2.58  &  ...  &  ...  &  <0  &  <0.52  &  <0.34  &  <0.86  &  <0.36  &  <0.88 \\
            3 &  J050632.10-714229.8  &  LMC  &  6750 $\pm$ 125  &  -1.22 $\pm$ 0.17  &  <2.05  &  <1.52  &  ...  &  ...  &  <0.45  &  <0.1  &  <0.80  &  <0.45  &  <0.84  &  <0.49 \\
            4 &  J052043.86-692341.0  &  LMC  &  5750 $\pm$ 125  &  -1.15 $\pm$ 0.17  &  <2  &  <1.4  &  ...  &  ...  &  <-0.45  &  <-0.27  &  <-0.15  &  <0.03  &  <-0.11  &  <0.07 \\
            5 &  J053250.69-713925.8  &  LMC  &  5500 $\pm$ 125  &  -1.22 $\pm$ 0.11  &  <2.23  &  <1.7  &  ...  &  ...  &  <-0.24  &  <0.19  &  <0.03  &  <0.46  &  <0.04  &  <0.47 \\
            7 &  J051213.81-693537.1  &  LMC  &  5875 $\pm$ 125  &  -0.56 $\pm$ 0.15  &  <3.3  &  <2.11  &  ...  &  ...  &  <0.37  &  <0.78  &  <0.47  &  <0.88  &  <0.49  &  <0.90 \\
            8 &  J051848.86-700246.9  &  LMC  &  6000 $\pm$ 125  &  -1.03 $\pm$ 0.14  &  <2.62  &  <1.93  &  ...  &  ...  &  <-0.19  &  <0.47  &  <0.09  &  <0.75  &  <0.14  &  <0.80 \\
            11 &  IRAS 05113+1347  &  Galaxy  &  5500 $\pm$ 125  &  -0.49 $\pm$ 0.2  &  <2.65  &  <1.44  &  ...  &  ...  &  <-0.21  &  <0.11  &  <-0.06  &  <0.26  &  <-0.05  &  <0.27 \\
            12 &  IRAS 05341+0852  &  Galaxy  &  6750 $\pm$ 125  &  -0.54 $\pm$ 0.2  &  <3.15  &  <2.1  &  ...  &  ...  &  <-0.14  &  <0.23  &  <0.12  &  <0.49  &  <0.15  &  <0.52 \\
            13 &  IRAS 06530-0213  &  Galaxy  &  7375 $\pm$ 125  &  -0.32 $\pm$ 0.2  &  <4.1  &  <2.73  &  <4.19  &  <2.76  &  <0.69  &  <0.98  &  <1.03  &  <1.32  &  <1.05  &  <1.34 \\
            14 &  IRAS 07134+1005  &  Galaxy  &  7250 $\pm$ 125  &  -0.91 $\pm$ 0.2  &  <2.79  &  <2.01  &  ...  &  ...  &  <0.38  &  <0.37  &  <0.75  &  <0.74  &  <0.78  &  <0.77 \\
            15 &  IRAS 07430+1115  &  Galaxy  &  6000 $\pm$ 125  &  -0.31 $\pm$ 0.2  &  <2.5  &  <1.07  &  ...  &  ...  &  <-0.48  &  <-0.23  &  <-0.32  &  <-0.07  &  <-0.32  &  <-0.07 \\
            16 &  IRAS 08143-4406  &  Galaxy  &  7000 $\pm$ 125  &  -0.43 $\pm$ 0.2  &  <3.2  &  <1.9  &  ...  &  ...  &  <0.32  &  <0.13  &  <0.61  &  <0.42  &  <0.64  &  <0.45 \\
            17 &  IRAS 08281-4850  &  Galaxy  &  7875 $\pm$ 125  &  -0.26 $\pm$ 0.2  &  <4.2  &  <2.74  &  <4.2  &  <2.71  &  <1.13  &  <1.14  &  <1.48  &  <1.49  &  <1.52  &  <1.53 \\
            19 &  IRAS 13245-5036  &  Galaxy  &  9500 $\pm$ 125  &  -0.26 $\pm$ 0.2  &  ...  &  ...  &  <4.4  &  <2.94  &  <0.91  &  <1.38  &  ...  &  ...  &  ...  &  ...    \\
            20 &  IRAS 14325-6428  &  Galaxy  &  8000 $\pm$ 125  &  -0.56 $\pm$ 0.2  &  ...  &  ...  &  <3.79  &  <2.6  &  <1.27  &  <1.35  &  ...  &  ...  &  ...  &  ...    \\
            21 &  IRAS 14429-4539  &  Galaxy  &  9375 $\pm$ 125  &  -0.64 $\pm$ 0.2  &  ...  &  ...  &  <4.4  &  <2.83  &  <1.36  &  <1.54  &  ...  &  ...  &  ...  &  ...    \\
            22 &  IRAS 19500-1709  &  Galaxy  &  8000 $\pm$ 125  &  -0.59 $\pm$ 0.2  &  <3.89  &  <2.72  &  ...  &  ...  &  <1.38  &  <1.35  &  <1.77  &  <1.74  &  <1.81  &  <1.78 \\
            24 &  IRAS 22223+4327  &  Galaxy  &  6500 $\pm$ 125  &  -0.3 $\pm$ 0.2  &  <3.25  &  <1.82  &  ...  &  ...  &  <0.94  &  <0.48  &  <1.14  &  <0.68  &  <1.16  &  <0.70 \\
            25 &  IRAS 22272+5435  &  Galaxy  &  5750 $\pm$ 125  &  -0.77 $\pm$ 0.2  &  <2.7  &  <1.72  &  ...  &  ...  &  <-0.18  &  <0.11  &  <0.02  &  <0.31  &  <0.05  &  <0.34 \\
            43 &  HD 168616  &  Galaxy  &  7250 $\pm$ 125  &  -0.64 $\pm$ 0.2  &  <2.75  &  <1.51  &  ...  &  ...  &  <0.59  &  <0.77  &  <0.92  &  <1.10  &  <0.96  & <1.14 \\
            \addlinespace
            \hline
        \end{tabular}
}
    \begin{tablenotes}
        \small
        \item \textbf{Notes:} All lead abundances and ratios, except for J003643, are upper limits derived using the SSF technique and have been adopted from \citet{desmedt2016} and \citet{Kamathuniverse2021}. \textcolor{green}{Details of NLTE TBA}
    \end{tablenotes}
    \label{tab:lead}
\end{sidewaystable}


